Few-Shot Unsupervised Image-to-Image Translation

Unsupervised image-to-image translation methods learn to map images in a given class to an analogous image in a different class, drawing on unstructured (non-registered) datasets of images. While remarkably successful, current methods require access to many images in both source and destination classes at training time. We argue this greatly limits their use. Drawing inspiration from the human capability of picking up the essence of a novel object from a small number of examples and generalizing from there, we seek a few-shot, unsupervised image-to-image translation algorithm that works on previously unseen target classes that are specified, at test time, only by a few example images. Our model achieves this few-shot generation capability by coupling an adversarial training scheme with a novel network design. Through extensive experimental validation and comparisons to several baseline methods on benchmark datasets, we verify the effectiveness of the proposed framework. Our implementation and datasets are available at https://github.com/NVlabs/FUNIT .

==> fig_animal_dataset.tex <==
\begin{figure}[!tbh]
	\centering
	\includegraphics[trim=0.00in 0.0in 0in 0in,width=0.49\textwidth] {figs/animal_dataset_small.pdf}
	\scaption{Illustration of the Animal Faces dataset. We show example images of 7 animal classes (out of 149 carnivorous animal classes) in our dataset. From top to bottom rows, the class names are Papillon, Labrador retriever, German shepherd, Persian cat, Leopard, Brown bear, and Meerkat.}
	\label{fig::animal_dataset}
\end{figure}

==> fig_interp.tex <==
\begin{figure}[t!]	
	\centering
	\includegraphics[trim=0in 0in 0in 0in,width=0.45\textwidth]{figs/interp1.jpg}
	\vspace{-1mm}
	\scaption{Interpolation by keeping the content code fixed while interpolating between two class codes of source classes. }
	\label{fig::interp}\vspace{-3mm}
\end{figure}

==> fig_prototypical.tex <==
\begin{table}[t!]
	\centering
	\small
    \resizebox{\columnwidth}{!}{
	\begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
		\hline 
		\multirow{3}{*}{\textbf{Method}} & \textbf{\# of} & \multicolumn{2}{c|}{\textbf{Average}}\\
		& \textbf{generated} & \multicolumn{2}{c|}{\textbf{Accuracy}}\\
		\cline{3-4}
		& {\bf samples} & {\bf Animal Faces} &{\bf N. A. Birds} \\
		\hline
		Prototypical Net.~[39] & 0 & 34.51 & 28.49 \\
		\hline
		Prototypical Net. & 10 & 40.07 & 33.63 \\
		$+$ & 50 & 39.85 & 33.74 \\
		{\proposed}& 100 & 40.47 & 34.28 \\
		\hline
	\end{tabular}%
	}
	\scaption{1-shot accuracies on the Animal Faces and the North American Birds datasets upon using generated images with the prototypical networks method~[39], averaged over 5 splits.}
	\label{tbl::prototypical}	

\end{table}
